Image-to-Image Translation for Autonomous Driving from Coarsely-Aligned Image Pairs

A self-driving car must be able to reliably handle adverse weather conditions (e.g., snowy) to operate safely. In this paper, we investigate the idea of turning sensor inputs (i.e., images) captured in an adverse condition into a benign one (i.e., sunny), upon which the downstream tasks (e.g., semantic segmentation) can attain high accuracy. Prior work primarily formulates this as an unpaired image-to-image translation problem due to the lack of paired images captured under the exact same camera poses and semantic layouts. While perfectly-aligned images are not available, one can easily obtain coarsely-paired images. For instance, many people drive the same routes daily in both good and adverse weather; thus, images captured at close-by GPS locations can form a pair. Though data from repeated traversals are unlikely to capture the same foreground objects, we posit that they provide rich contextual information to supervise the image translation model. To this end, we propose a novel training objective leveraging coarsely-aligned image pairs. We show that our coarsely-aligned training scheme leads to a better image translation quality and improved downstream tasks, such as semantic segmentation, monocular depth estimation, and visual localization.

==> figurestext/largefig.tex <==
\begin{figure*}[t]%TRIM: left, lower, right, upper
    \begin{minipage}{0.48\linewidth}
        \centering %TRIM: left, lower, right, upper
        \includegraphics[width=\linewidth]{figures/INTRO-FIGURE.png}
      \caption{\small Left: perfectly-aligned pair from Apollo \emph{Synthetic} dataset~\cite{huang2018apolloscape}. Mid: coarsely-aligned pair from multiple traversals in Ithaca365 dataset~\cite{diaz2022Ithaca365}. Right: unaligned images~\cite{diaz2022Ithaca365}.\label{fig:intro}}
    \end{minipage}\hfill %\hspace{5pt}
    %******************
    \begin{minipage}{0.48\linewidth}
        \centering\vspace*{-0.1 in}
        %0.4/0.58 line width
        %\includegraphics[width=1\linewidth, trim={0cm 4cm 1cm 3cm},clip]{figures/Approach-Figure.old.png}
        \includegraphics[width=1\linewidth]{figures/Approach-Figure.png}
        \caption{\small \ourmethod framework for training image translation model $G$ using coarsely-aligned image pairs.\label{fig:diagram}}
    \end{minipage}

    \vskip -8pt
    \label{fig:example}
\end{figure*}

==> sec/method.old.tex <==
\section{Proposed Approach: \ourmethod}
% \subsection{Problem Setup} We aim to learn a mapping function $G$ from a source image domain $\sX$ (\eg, adverse weather like snowy) to a target image domain $\sY$ (\eg, sunny). We assume that we have two set of training images $X = \{x^{(n)}\}_{i=1}^N$ and $Y = \{y^{(n)}\}_{i=1}^N$ from both domains.and they can be paired into $\{(x^{(n)}\in\sX, y^{(n)}\in\sY)\}_{i=1}^N$. Each paired images are taken from close-by locations but are \emph{not perfectly aligned} due to potential GPS differences/errors, different semantic layouts due to different collection time, and shifts in camera poses, etc. For example, the Ithaca365 dataset~\cite{} collects images and GPS on the same route under different weather conditions (\eg, sunny, night, snowy). We pair images from different traversals based on closest GPS poses. See Figure~\ref{xx} for some example training data. 
\subsection{Problem Setup}
Our goal is to learn an image mapping function $G$ from a source domain $\mathcal{X}$ (\eg, adverse weather) to a target domain $\mathcal{Y}$ (\eg, sunny). We assume two set of training images $X = \{x^{n}\}_{n=1}^N \in \mathcal{X}$ and $Y=\{y^n\}_{n=1}^N \in \mathcal{Y}$ from both domains. In many scenarios, it is infeasible to obtain paired images. However, in autonomous driving application, we can still obtain \textit{coarse} pairs $\{(x^n\in\mathcal{X}, y^n\in\mathcal{Y})\}_{n=1}^N$ if they are collected from the same route/ area. 
%For instance, we can pair two images if their GPS locations are close-by; we note that these paired images are \emph{not perfectly aligned} due to potential GPS differences/errors, changes in semantic layouts at different collection times, and shifts in camera pose.
For example, the Ithaca365 dataset~\cite{diaz2022Ithaca365} collects images and GPS on the same route under different weather conditions (\eg, sunny, night, and snowy). Therefore, we pair images from different traversals 
based on the closest GPS poses (see \autoref{fig:intro}-mid for a training data sample). We note that these paired images are \emph{not perfectly aligned} due to potential GPS differences/errors, changes in semantic layouts at different collection times, and shifts in camera pose. 

We train $G$ using a GAN-style loss~\cite{isola2017image,CycleGAN2017}. However, instead of directly employing the paired translation algorithms~\cite{isola2017image} or entirely ignoring the paired information by applying an unpaired algorithm~\cite{CycleGAN2017}, we propose \ourmethod, which is dedicated to learning image translation using \textit{coarsely-aligned} image pairs. 

\subsection{Baseline Algorithm} 
\label{ss_baseline}
To begin with, let us introduce a baseline paired translation algorithm, inspired by~\cite{isola2017image}. \cite{isola2017image} assumes that the training data are perfectly paired images, and introduces an L1 loss comparing paired images $x^{n}$ and $y^{n}$ in pixel space.
\begin{equation}
    \mathcal{L}_{L1}(G) = \mathbb{E}_{(x,y)\sim(X,Y)}\lVert  G(x) - y \rVert_1
\end{equation}
%\begin{equation}
%    \mathcal{L}_\text{1}(G,X,Y) = \frac{1}{N}\sum_n\frac{1}{K^{n}}\sum_{i,j} \|G(x^{n})_{i,j} - y^{n}_{i,j}\|_1.\label{e_L1}
%\end{equation}
Here, $G(x^{n})_{i,j}$ and $y^{n}_{i,j}$ are the pixel values at the $(i,j)$ location and $K^{n}$ is the number of pixels in image $y^{n}$. %We empirically find that L1 loss is still quite effective in learning with coarsely-aligned data.

% In~\cite{isola2017image}, $D$ is designed to tell a real source-target pair $(x^{(n)}, y^{(n)})$ from the corresponding fake pair $(x^{(n)}, G(x^{(n)}))$, taking advantage of the perfectly aligned image pairs. 

Along with the L1 loss, \cite{isola2017image} further employs a GAN loss~\cite{goodfellow2014generative}. Let $D$ denotes a discriminator (\ie, binary classifier) that tells a real image $y\in\mathcal{Y}$ from a fake, generated one $G(x)$, where $x\in\mathcal{X}$. 
The GAN loss~\cite{goodfellow2014generative} can be defined as follows:
%\begin{equation}
\begin{multline}
    \mathcal{L}_\text{GAN}(G,D) = \\ \mathbb{E}_{y\sim Y}\left[\log D(y)\right] +  \mathbb{E}_{x\sim X}\left[\log \left(1-D(G(x))\right)\right].\label{e_baseGAN}
\end{multline}
%\end{equation}
Through minimizing both losses with respect to $G$, we encourage the generated images to look real and similar to the target images\footnote{\autoref{s_exp} provides a study to compare different designs of $D$.}.
% We note that in~\cite{isola2017image}, $D$ is designed to tell a real source-target pair $(x^{(n)}, y^{(n)})$ from the corresponding fake pair $(x^{(n)}, G(x^{(n)}))$. FOOTNOTE

% Let us denote by $D$ a discriminator (\ie, binary classifier), which is used to tell a real image from a fake, generated one. In~\cite{isola2017image}, $D$ is designed to tell a real source-target pair $(x^{(n)}, y^{(n)})$ from the corresponding fake pair $(x^{(n)}, G(x^{(n)}))$, taking advantage of the perfectly aligned image pairs. In this paper, since $(x^{(n)}, y^{(n)})$ is only coarsely-aligned, we follow~\cite{CycleGAN2017} to train  $D$ to differentiate $y\in\sY$ from $G(x)$, where $x\in\sX$. We then define the GAN loss~\cite{goodfellow2014generative} as follows\footnote{We provide ablation study in section~\ref{s_exp} to compare different input designs to $D$.}

\begin{figure}[t]%TRIM: left, lower, right, upper
  \centering 
\includegraphics[width=1\linewidth, trim={0cm 4cm 0 3cm},clip]{figures/Approach-Figure.png}
\caption{Illustration of our proposed approach: \ourmethod. We aim to train an image-to-image translation model $G$ using coarsely-aligned image pairs.\label{fig:diagram}} 
\vskip -8pt
\end{figure}
% CAPTION:Given two image domains (\eg, night vs. sunny) and coarsely-aligned image pairs, we aim to train an image-to-image translation model $G$. Besides the GAN loss using a discriminator $D$, we propose two novel loss terms: masked misalignment-tolerating L1 loss that compares one pixel to a window of nearby pixels, and masked patchNCE loss that compares generated image patches to target image patches to overcome stochastic, large misalignment.

\subsection{Learning with Coarsely-Paired Images}
\label{ss_loss}
Learning with the above two loss functions does not explicitly account for the misalignment in the coarsely-aligned image pairs and may adversely degrade the resulting generative model. One obvious solution is to apply unpaired translation algorithms~\cite{CycleGAN2017,huang2018munit}, which, however, entirely ignore any useful paired information in the training data. To address these challenges and drawbacks, we propose novel loss functions tailored to coarsely-aligned image pairs.

\subsubsection{Foreground-Masked Loss}
Our first insight about the coarsely-aligned data is that, unlike stationary backgrounds, foreground objects (\eg, cars and pedestrians) change in presence and location over time. Thus, two images taken at different timestamps mostly have different foreground contents and layouts, even if they are taken from exactly the same camera pose. To address this issue, we propose to mask out pixels of the foreground objects in calculating any paired loss (\eg, the L1 loss). For example, we only calculate the L1 loss on pixels that belong to the backgrounds in both the source and the corresponding target images. Let us denote the background pixel indices as $M(x,y)$:
\begin{align}\label{eq:fgmask}
    M(x,y)=\{(i,j) | c(x_{i,j}) \not\in \text{fg} \wedge c(y_{i,j})\not\in \text{fg}\}, 
\end{align}
where $c(\cdot)$ denotes the label of a pixel; fg means the set of foreground classes. We can segment these objects using annotated masks or via off-the-shelf segmentation models~\cite{he2017mask}.

\subsubsection{Misalignment-Tolerating L1 Loss}
The original L1 loss penalizes differences in pixel values between the generated image and the target image at each pixel location. 
%In other words, it assumes that the two images are perfectly aligned. 
However, with coarsely-aligned data, the source and target images are unlikely from the exact same camera poses. Thus, a conventional L1 loss would exaggerate even with just a few pixel shifts between the two images (\eg, along the edges), adversely forcing the generator to fit noises. 
To address this problem, we propose to compare $G(x)_{i,j}$ not just to $y_{i,j}$ as in \autoref{e_L1}, but to a set of pixels within a small rectangle window around $i,j$. Specifically, we refer to those pixel indices as
\begin{equation}\label{eq:k}
    r(i,j)=\{(a,b):  |a-i|\leq k_H \wedge |b-j|\leq k_W \}
\end{equation}
,where $k_H$ and $k_W$ are the size of the rectangular window. With this window, given $x_{i,j}$ we then first find the best corresponding pixel in $y$ to overcome the slight pixel-to-pixel misalignment. The misalignment-tolerating L1 loss can be formulated as:
%\begin{equation}
\begin{multline}
    \mahthcal{L}_1^{\dagger}(G) = \frac{1}{N}\sum_n\frac{1}{K^{n}}\sum_{i,j} \min_{(i',j')\in r(i,j)} \lVert G(x^{n})_{i,j}-y^{n}_{i',j'}\rVert_1. \label{e_new_L1}
\end{multline}
%\end{equation}
\autoref{e_new_L1} can be further combined with the foreground masking defined in \autoref{eq:fgmask} into the final L1 loss:
%\begin{align}
%    & \mathcal{L}_1^{\star}(G) = \nonumber \\
%    & \frac{1}{N}\sum_n\frac{1}{|M^{n}(x,y)|}\sum_{(i,j)\in M^{n}(x,y)} \min_{(i',j')\in r(i,j)\cap M^{n}(x,y)} \lVert G(x^{n})_{i,j}-y^{n}_{i',j'}\rVert_1.
%\end{align}
\begin{align}
    & \mathcal{L}_1^{\star}(G) = \nonumber \\
    & \mathbb{E}_{(x,y)\sim(X,Y)} \mathbb{E}_{(i,j)\sim M(x,y)} \min_{(i',j')\in \{r(i,j)\cap M(x,y)\}} \lVert G(x)_{i,j}-y_{i',j'}\rVert_1.
\end{align}
% NCE LOSS
\subsubsection{Ranking-based Loss to Overcome Large, Stochastic Variations}
The misalignment-tolerating L1 loss can effectively compensate for small pixel shifts due to different camera poses. However, even if two images are from the same camera pose and the foreground objects are masked out, the fact that the two images are captured at different time implies that there are inevitable \emph{stochastic} factors that could affect the image contents and cause large misalignment. For example, the same tree might be posed differently due to the wind, which in turn can cause different shadow patterns on the sidewalks. These stochastic variations could significantly distort the pixel values, which cannot be alleviated by the misalignment-tolerating L1 loss.


%We resort to a retrieval-style loss. In image retrieval --- \eg, given an image of Golden Gate Bridge, retrieve other images of Golden Gate Bridge from an image collection --- the stochastic variations or large misalignment are more or less assumed among different Golden Gate Bridge images. Consequently, instead of learning to minimize the distance among images, image retrieval mainly asks to rank semantically similar images with a higher feature similarity than semantically dissimilar images, so they can be retrieved first.

To address these stochastic variations, we propose to employ a paired loss term beyond minimizing the differences at same pixel locations. Concretely, we build upon a key insight --- while there exist stochastic variations, patches of the generated and target images at the same position should capture similar structures and contents, such that their similarity are larger than patches at different positions. We realize this idea using a loss similar to the patchNCE loss \cite{park2020contrastive}\footnote{\cite{park2020contrastive}, being an unpaired translation algorithm, computes the patchNCE loss between the source and translated images. However, we compute the patchNCE loss between the translated and coarsely-aligned target images.}. 
Let $H$ be a feature extractor and $H_s$ be the feature at the spatial location $s$ on the feature map, our usage of the patchNCE loss is defined as follows:
\begin{equation}
\begin{split}
     \sum_s \ell\left(H_s(G(x)), H_s(y), \{H_{s'}(y) | s'\neq s\}\right), \\
    \text{where } \ell(v,v^{+}, \{v^{-}_{s'}\})=\\
    -\log\left[\frac{\exp(v\cdot v^{+}/\tau)}{\exp(v\cdot v^{+}/\tau)+\sum_{s'} \exp(v\cdot v^{-}_{s'}/\tau)}\right].
\end{split}
\end{equation}

Here, $\tau$ is a temperature constant scalar. Through minimizing this loss with respect to $G$, we encourage $H_s(G(x))$ and $H_s(y)$ to have higher inner product similarity than $H_s(G(x))$ and other patches of $y$. By applying this loss to all the training pairs, we have
\begin{multline}
    \mathcal{L}_\text{patchNCE}(G,H)=\\ \frac{1}{N}\sum_s \ell\left(H_s(G(x^{n})), H_s(y^{n}), \{H_{s'}(y^{n}) | s'\neq s\}\right).
\end{multline}

Our implementation follows~\cite{park2020contrastive} to extract features from multiple layers. Furthermore, we apply $M(x,y)$ to mask out the foreground objects. 

\subsection{Final \ourmethod Training Objective}
Combining the GAN loss with the loss terms introduced in \autoref{ss_loss}, our \ourmethod training objective is:
\begin{equation}
    \mathcal{L}_\text{GAN}(G,D) + \lambda_1 \mathcal{L}_\text{patchNCE}(G,H)+ \lambda_2 \mathcal{L}_1^\star(G).
\end{equation},
where $\lambda_1$ and $\lambda_2$ are weighting coefficients.
Specifically, we learn $G$ and $H$ to minimize the objective, while $D$ to maximize the objective.

\subsection{Implementation and Training Detail}
\ourmethod is in theory agnostic to different model architectures of the generator $G$ and the discriminator $D$. In this paper, we adopt a coarse-to-fine generator $G$ and a multi-scale discriminator $D$ from the Pix2pixHD \cite{wang2018high}.
For training, we use mini-batch stochastic gradient descent with a learning rate of $0.0002$ for the first $50$ epochs and linearly decrease the learning rate to $0$ in the next $50$ epochs. 
%For the remaining $50$ epochs, the learning rate linearly decreases to zero. 
We use Adam optimizer~\cite{kingma2014adam} with $\beta_{1}=0.5$ and $\beta_{2}=0.999$.
%In addition, we use Adam optimizer~\cite{kingma2014adam} for both the generator and the discriminator, the $\beta_{1}$ is $0.5$ and $\beta_{2}$ is $0.999$ for the utilized Adam optimizer. Finally, we train our proposed methodology on one NVIDIA RTX3090 for $100$ epochs using the Ithaca365 dataset~\cite{diaz2022Ithaca365}.
%%%%%%%%%%%%%% OLD TEXT %%%%%%%%%%%%%

%Our goal is to learn a mapping from  driving scene images in adverse condition domain $\mathcal{X}$ (i.e., snowy and night) to appear like in the ideal condition domain $\mathcal{Y}$ (i.e., sunny). We use a GAN-based image translation model, specifically we adopt a corase-to-fine generator $G$ and a multi-scale discriminator $D$ from the Pix2pixHD \cite{wang2018high} architecture.

%Exact paired correspondences between $\mathcal{X}$ and $\mathcal{Y}$ are not available for real driving data, forcing existing work to train in a more challenging unpaired image translation setting without paired supervision. However, although exact paired correspondences between $\mathcal{X}$ and $\mathcal{Y}$ are not available for real driving data, we can still obtain \emph{coarsely}-paired image pairs as follows. Given driving data (images and corresponding GPS poses) collected on the same route under different conditions (e.g., sunny, night, snowy), we pair images based on closest GPS poses \color{red}See Figure xxx\color{black}. This results in two sets of images $X=\{x^i\}_{i=1}^{N}\subset \mathcal{X}$ and $Y=\{y^i\}_{i=1}^N\subset\mathcal{Y}$ where $x^i$ is \emph{coarsely} aligned to $y^i$.

% Our key idea is to exploit the \emph{coarse} correspondence for extra supervision during training. Specifically, we employ two reconstructive losses, i.e., L1 \cite{isola2017image} and patchNCE \cite{andonian2021contrastive} between translated image $G(x)$ and \emph{coarse} target image $y$. However, since our image pairs are not well aligned, we propose a simple but effective approach to adapt the use of reconstructive losses, originally designed for paired images, to \emph{coarsely}-paired images. This allows us to train image translation models with some supervision from \emph{coarsely}-paired images despite the unavailability of exact paired images. 

%The original L1 loss penalizes distance between target image and output image, encouraging the output to be near target image. As the target image aligns with the input image, this also encourages that the output image respects the input image. L1 works under the assumption that the input image and its target correspondence are perfectly aligned. Although our image pairs have been \emph{coarsely}-aligned using GPS poses, there are still several key factors that can degrade the performance.

\iffalse
First, unlike stationary backgrounds and structures, foreground objects (e.g., cars and pedestrians) change in terms of locations and presence over time. Thus, two images taken at different time instances will have different foreground content even if they are taken from exactly the same global pose. To address this issue, we propose to calculate L1 only on pixel locations whose semantic in both input $x$ and coarse target image $y$ are not foreground. Specifically, we refer to the pixel indices as $M(x,y)$:
\begin{equation}
    M(x,y)=\{(i,j):  0<i<H \wedge 0<j<W \wedge c(x_{ij}) \not\in \text{fg} \wedge c(y_{ij})\not\in \text{fg}\}
\end{equation}, where $c(\cdot)$ denotes semantic label of a pixel, fg means foreground, and $H,W$ are the height and width dimension of the images.
%Specifically, let $M(z)$ be a set of pixel index locations $(i,j)$ on some image $z$ where pixel $z_{ij}$ has non-foreground semantic class. We compute L1 loss only on $M(x) \cap M(y)$ indices whose pixels belong to non-foreground semantic class in both input image $x$ and its corresponding coarse target image $y$. 
\fi

\iffalse
Second, while image pairs are matched based on closest GPS poses, they do not come from the same exact pose. Mainly, this is because it is practically impossible to drive on the same exact poses under two different collection drives. Furthermore, GPS also has some inherent error. Thus, image misalignment between the \emph{coarsely}-paired images is inevitable. While the misalignment may be small for some cases, but the impact to L1 may be significant. Concretely, even several pixels shift in image may cause very different change in pixel values, especially on object boundaries. Hence, comparing pixel $G(x)_{ij}$ in the output image to \emph{strictly} $y_{ij}$ in the \emph{coarse} target image may not be appropriate, as pixel $x_{ij}$ may correspond to other nearby pixel $y_{i'j'}$ instead of $y_{ij}$. To this extent, we propose to compare $G(x)_{ij}$ to a set of pixels within a small rectangle window around $y_{ij}$. Specifically, we refer to those pixel indices as:
\begin{equation}
    n(ij)=\{(a,b):  |a-i|<k_H \wedge |b-j|<k_W \wedge 0<i<H \wedge 0<j<W\}
\end{equation}
where $k_H$ and $k_W$ defines the size of the rectangular window. This is to address the slight pixel-to-pixel correspondence misalignment.

Overall, the final L1 loss can be formally expressed as:
\begin{equation}
    \mathcal{L}_1^*(G,X,Y) = \mathbb{E}_{x\sim X}\frac{1}{|M(x,y)|}\sum_{(i,j)\in M(x,y)} \min_{(i',j')\in n(ij)\cap M(x,y)} \lVert G(x)_{ij}-y_{i'j'}\rVert_1
\end{equation}
\fi

\iffalse
\subsubsection{Adapting patchNCE Loss}
patchNCE loss \cite{park2020contrastive}, originally proposed for unpaired image translation, aims to regulate output image to preserve basic structure and content from the input image in a patch-wise way. Specifically, it encourages a patch in the translated image to be more similar (in content) to the corresponding patch in the input image, relative to other patches from the input image. It uses contrastive learning framework, formulated as a $N+1$-way classification problem, where the probability that a query $v$ matches with positive sample $v^{+}$ over negatives \{$v^{-}_{n}\}_{n=1}^N$ is represented by cross-entropy loss:
\begin{equation}
    \ell(v,v^{+},v^{-})=-\log\left[\frac{\exp(v\cdot v^{+}/\tau)}{\exp(v\cdot v^{-}/\tau)+\sum_{n=1}^{N}\exp(v\cdot v^{-}_{n}/\tau)}\right]
\end{equation}
where $\tau$ is a temperature constant scalar.

Original patchNCE loss uses features extracted from patches in input image as negative and positive samples. However, since we have \emph{coarsely}-paired images, we can directly use the patchNCE loss between the output image $G(x)$ and its \emph{coarse} coarse correspondence $y$ from the target domain. Unlike L1, small misalignment in image should not degrade the optimality of patchNCE, because contrastive learning does not force strict equality. However, we still need to account for foreground objects difference. Thus $\neg M(x,y)$ pixels are masked in both output and target images for patchNCE loss computation.

Following \cite{park2020contrastive}, features are extracted from $L$ selected layers of interest using the encoder part of our generator $G_\text{enc}$ and two-layer MLP networks.
Specifically, MLP network $H_l$ is used for the output of the $l$-th chosen output layer from $G^l_\text{enc}$, resulting in stacks of features $q_l=H_l(G_\text{enc}^l(G(x)))$ and $w_l = H_l(G_\text{enc}^l(y))$ from output and target images respectively. These features are used for pathNCE loss computation:
\begin{equation}
    \mathcal{L}_\text{patchNCE}(G,H,X,Y)=\mathbb{E}_{x\sim X}\sum_{l=1}^{L}\sum_{s=1}^{S_l}\ell(q_{l}^{s},w_{l}^{s},w_{l}^{S\setminus s})
\end{equation}
, where $s \in \{1, \dots, S_l\}$ denotes the spatial location, marking $q_l^s$ and $w_l^s$ as corresponding features, and $q_l^{S\s}$ as features from other non-corresponding locations. This encourages maximum mutual information between the generated image and the reference image. $ q_l^s$ and $w_l^s$ are corresponding features at the $s$-th spatial location and $l$-th layer
\color{red}talk about s and $S/s$\color{black}
% GAN LOSS
\fi

\iffalse
\subsection{Generative Adversarial Loss}
Generative adversarial loss \cite{goodfellow2014generative} is used to encouraged generated images to look similar to images in target domain:
\begin{equation}
    \mathcal{L}_\text{GAN}(G,D,X,Y) = \mathbb{E}_{y\sim Y}\left[\log D(y)\right] + \mathbb{E}_{x\sim X}\left[\log \left(1-D(G(x))\right)\right]
\end{equation}
As we employ Pix2pixHD \cite{wang2018high} architecture which contains multi-scale discriminator, the GAN loss above is applied at every scale of the discriminator.


%While paired images are desired to enable supervision using reconstructive loss, we empirically find that feeding unpaired images of real and fake images for the GAN loss results in better performance than feeding paired real and fake images. Thus, we feed unpaired images for the GAN loss. \color{red}Add explanation why better: discriminator\color{black}
%\color{red}Talk that existing work for paired translation feed paired images for GAN loss\color{black}
\fi



==> tables/several.tex <==
% https://tex.stackexchange.com/questions/271347/minipage-across-two-columns
% Minipage alignment https://tex.stackexchange.com/questions/69560/what-is-the-best-way-of-arranging-multiple-minipages-on-a-page
\setlength{\tabcolsep}{1pt}
\begin{figure*}
%\tiny
%\captionsetup{justification=centering}
  \begin{minipage}{.53\textwidth}
   \captionof{table}{Evaluation of \ourmethod Vs other unpaired translation methods through FID and several downstream tasks on the Ithaca365 dataset.}\vspace{2pt} %semantic segmentation (PixAcc), and depth estimation ($\delta<1.25$).
    \label{table:comparison-all}
    \begin{tabular}{cccccc}
        \hline
        No & Method & FID$\downarrow$ & PixAcc (\%)$\uparrow$ & $\delta<1.25$ (\%)$\uparrow$ & loc-err(m)$\downarrow$\\ 
        \hline \noalign{\smallskip}
        1. & No adaptation &  162.4 / 165.2  & 50.9 / 68.4    & 70.7  / 74.5 & 22.5 / 12.1\\
        \noalign{\smallskip} \hdashline \noalign{\smallskip}
        2. & CycleGAN        & 158.3 / 136.9 & 52.8 / 64.2    & 78.3 / 73.8 & 9.3 / 5.7\\
        3. & MUNIT           & 96.3 / 162.4 & 47.4  / 58.8    & 77.0  / 67.1 & 10.8 / 7.9\\
        4. & ACL-GAN        & 89.4 / 101.1 & 48.0  / 68.5    & 77.0 / 73.0 & 11.2 / 6.6\\
        5. & CUT             & 94.0 /  99.2 & 53.8 / 67.8    & 79.5   / 75.8 & 9.3 / 5.0\\
        6. & ToDayGAN & 83.2 / 87.8 & 57.4 / 73.5 & x / x & 8.9 / 3.4\\
        7. & ForkGAN & 80.9 / 101.2 & 54.2 / 68.7 & x / x & 8.8 / 5.36\\ 
        8. & \ourmethod (ours)            & \textbf{69.4} / \textbf{76.2} & \textbf{61.9} / \textbf{75.2}     & \textbf{83.0} / \textbf{76.8} & \textbf{6.3} / \textbf{2.9}\\ 
        \noalign{\smallskip}
        \hdashline
        \noalign{\smallskip}
        9. & Real sunny      & 60.1   & 89.2     & 88.5 & 2.2 \\
        \hline
    \end{tabular}

  \end{minipage} 
  \hfill%\hspace{2pt}
\begin{minipage}{0.45 \textwidth}
\captionof{table}{Ablation study of different loss functions.\label{table:ablation}}
\begin{tabular}{lc}
    \hline\noalign{\smallskip}
    Loss & FID $\downarrow$ \\
    \noalign{\smallskip}
    \hline
    cGAN + L1        & 114.0 / 122.1 \\ 
    cGAN + L1(+mask)         & 106.9 / 119.8  \\
    uGAN + L1(+mask)    & 94.8 / 114.8\\
    uGAN + L1(+mask) + NCE (+mask)   & 68.5 / 86.6\\
    uGAN + L1(+mask + misalignment) + NCE(+mask)        & 69.4 / 76.2 \\
    \hline
\end{tabular}
\end{minipage}
\end{figure*}
\setlength{\tabcolsep}{1.4pt}

